Evaluate-and-Purify: Fortifying Code Language Models Against Adversarial Attacks Using LLM-as-a-Judge

The widespread adoption of code language models in software engineering tasks has exposed vulnerabilities to adversarial attacks, especially the identifier substitution attacks. Although existing identifier substitution attackers demonstrate high success rates, they often produce adversarial examples with unnatural code patterns. In this paper, we systematically assess the quality of adversarial examples using LLM-as-a-Judge. Our analysis reveals that over 80% of adversarial examples generated by state-of-the-art identifier substitution attackers (e.g., ALERT) are actually detectable. Based on this insight, we propose EP-Shield, a unified framework for evaluating and purifying identifier substitution attacks via naturalness-aware reasoning. Specifically, we first evaluate the naturalness of code and identify the perturbed adversarial code, then purify it so that the victim model can restore correct prediction. Extensive experiments demonstrate the superiority of EP-Shield over adversarial fine-tuning (up to 83.36% improvement) and its lightweight design 7B parameters) with GPT-4-level performance.

==> table.tex <==
\begin{table*}[h]
    \centering
    \caption{Performance comparison of variants on the Beibei dataset. }
    \begin{threeparttable}
        % \setlength{\tabcolsep}{7mm}{
        \resizebox{\textwidth}{!}{
            \begin{tabular}{c|cccc cccc}
            \toprule [1.2pt]%设置线宽
            
            Variant &HR@10 &NDCG@10 &HR@20 &NDCG@20 &HR@50 &NDCG@50   \\
            \hline

            c/cart-buy &0.0963	&0.0481	&0.1534	&0.0625	&0.2558	&0.0827	\\
            
            c/view-buy &0.1030	&0.0506	&0.1586	&0.0646	&0.2591	&0.0845	\\
            \hline
           
            e/all &0.1046	&\textbf{0.0538}	&0.1641	&0.0688	&0.2635	&0.0885	\\
            
            e/view &0.0848	&0.0423	&0.1421	&0.0567	&0.2682	&0.0815	\\
            
            e/cart &\textbf{0.1060}	&0.0522	&\textbf{0.1735}	&\textbf{0.0691}	&\textbf{0.3080}	&\textbf{0.0957}	\\
            
            e/buy &0.1012	&0.0512	&0.1651	&0.0673	&0.2688	&0.0878	\\
            
            \bottomrule [1.2pt]
            \end{tabular}
            }
    \end{threeparttable}
    \label{tab:val}
\end{table*}
